An Integrity-Focused Threat Model for Software Development Pipelines

In recent years, there has been a growing concern with software integrity, that is, the assurance that software has not been tampered with on the path between developers and users. This path is represented by a software development pipeline and plays a pivotal role in software supply chain security. While there have been efforts to improve the security of development pipelines, there is a lack of a comprehensive view of the threats affecting them. We develop a systematic threat model for a generic software development pipeline using the STRIDE framework and identify possible mitigations for each threat. The pipeline adopted as a reference comprises five stages (integration, continuous integration, infrastructure-as-code, deployment, and release), and we review vulnerabilities and attacks in all stages reported in the literature. We present a case study applying this threat model to a specific pipeline, showing that the adaptation is straightforward and produces a list of relevant threats.

==> chapters/tab_old_threats_deploy_pipeline.tex <==
\begin{table}[h!]
\centering
\caption{Summary of threats and mitigations found for the deployment pipeline}
\label{tab:summary_model_bass}
\def\arraystretch{1.3}
\scalebox{0.85}{
\begin{tabular}{|p{4cm}|p{2cm}|p{3.5cm}|p{4.5cm}|p{1cm}}
    \cline{1-4}
    \multicolumn{1}{|c|}{\textbf{Diagram element}} & \multicolumn{1}{c|}{\textbf{Threat type}} & \multicolumn{1}{c|}{\textbf{Threat}} & \multicolumn{1}{c|}{\textbf{Mitigation}} &  \\ \cline{1-4}
    \multirow{3}{*}{\begin{minipage}{4cm}Continuous Integration, Test, Deployer, AWS OpsWorks, and Download/App Server\end{minipage}} & \textit{Spoofing} & Server spoofing & TLS certificates &  \\ \cline{2-4} & 
        \multirow{2}{*}{\textit{Tampering}} & Receiving unreliable data & Image checksum, encryption and obfuscation data &  \\ \cline{3-4} &  & Local spoofing & AWS OpsWorks mechanisms, restricted access to resources &   \\ \cline{1-4}
   
    \multirow{1}{*}{Data flows (all)} & \textit{Tampering} & Changing data during communication & TLS cryptography &  \\ \cline{1-4} 
   
    \multirow{1}{*}{\begin{minipage}{4cm}Application Code storage, Image Storage, and Binary Repository\end{minipage}} & \begin{minipage}[t][2cm][t]{2cm}\textit{Tampering} \end{minipage}& Improper data alteration & Manage access permissions and encrypt the data before storing it &  \\ \cline{1-4}  
\end{tabular}
}
\end{table}


